PACO: Parts and Attributes of Common Objects

Object models are gradually progressing from predicting just category labels to providing detailed descriptions of object instances. This motivates the need for large datasets which go beyond traditional object masks and provide richer annotations such as part masks and attributes. Hence, we introduce PACO: Parts and Attributes of Common Objects. It spans 75 object categories, 456 object-part categories and 55 attributes across image (LVIS) and video (Ego4D) datasets. We provide 641K part masks annotated across 260K object boxes, with roughly half of them exhaustively annotated with attributes as well. We design evaluation metrics and provide benchmark results for three tasks on the dataset: part mask segmentation, object and part attribute prediction and zero-shot instance detection. Dataset, models, and code are open-sourced at https://github.com/facebookresearch/paco.

==> intro_dhruv.tex <==
\section{Introduction}
\label{sec:intro}

With the significant advances in the field of multi-modal understanding~\cite{} and Generative adversarial Networks (GANs)~\cite{}, 
fine-grained semantic understanding of the visual scenes is becoming more and more important. Multi-task Visual-Language models~\cite{} that can perform variety of tasks like zero-shot recognition, captioning, visual question answering, etc. are becoming increasingly popular.  Object or scene level descriptions are not enough anymore. Models now need to understand and describe objects and scenes in terms of fine-grained parts and their attributes (colors, patterns, etc.).  In addition, with increasing emphasis on Explainable machine learning, models that can explain their predictions based on parts and attributes~\cite{} and glass-box models~\cite{} that directly base their predictions on parts and attributes are becoming very popular. As a result, going  beyond segmentation of object and scenes towards denser annotations of their parts and attributes is becoming increasingly important.

Current datasets with parts or attributes annotations have several shortcomings. Most datasets that have part-segmentation annotations are very small in size. ADE20K~\cite{} which is a  popular part-level dataset has only $20.5K$ images. In addition, most of these datasets are object-centric, objects are very large and in the center of the image. Hence, these datasets do not depict real-world scenarios where objects are present in very diverse settings and parts can be of low to medium resolution. On the attributes side, there exists large-scale datasets like Visual Genome~\cite{}, GQA~\cite{} that have object level attributes. However, with the exception of very small-scale datasets limited to fine-grained classes (for example, birds, dogs), none have any part-level attribute annotations. 

In this paper we introduce a new large-scale parts and attributes dataset \dataname to address the above mentioned limitations. \datname consists of around $83.5k$ images across $75$ entities commonly found in the household settings. Images are sourced from two datasets from diverse domains: a) LVIS~\cite{} which is currently a popular benchmark for object level detection and segmentation, and, b) Ego4D~\cite{} which is a recently released large scale ego-centric dataset. Our dataset has both object-centric and scene-centric images. \dataname has more than $300k$ part-level segmentation annotations for $200$ parts, an order of magnitude more than what any dataset has. In addition, we also provide annotations for $30$ different attributes for parts and objects for a subset of images. These attributes range from color, patterns, materials to logos and text and are chosen via careful user study of the instance recognition tasks. In addition, we also provide around $19k$ object instance level annotations. The main difference from existing datasets are: scale, diversity, part-level attribute annotations and instance level annotations.

Finally, we also provide five associated benchmark tasks on \dataname to help the community evaluate its progress over time. These tasks include: a) basic part segmentation and attribute prediction evaluation, b) applications like zero-shot recognition (textual queries) and few-shot instance recognition (visual queries), and, c) benchmarking of glass-box models~\cite{} in the Explainable AI domain. We believe that it is crucial to set-up benchmarks beyond standard segmentation evaluation for parts because unlike objects, part boundaries may not be very well defined (for example, for birds, it is not clear where neck ends and breast starts). Hence, it is crucial to evaluate the quality of the parts segmentation and prediction by the impact on the downstream applications. Code for the training and evaluation on these tasks along with some base models are provided as part of the release\footnote{https://releasedataset.com}.


